Eating Habits Discovery in Egocentric Photo-streams

Eating habits are learned throughout the early stages of our lives. However, it is not easy to be aware of how our food-related routine affects our healthy living. In this work, we address the unsupervised discovery of nutritional habits from egocentric photo-streams. We build a food-related behavioural pattern discovery model, which discloses nutritional routines from the activities performed throughout the days. To do so, we rely on Dynamic-Time-Warping for the evaluation of similarity among the collected days. Within this framework, we present a simple, but robust and fast novel classification pipeline that outperforms the state-of-the-art on food-related image classification with a weighted accuracy and F-score of 70% and 63%, respectively. Later, we identify days composed of nutritional activities that do not describe the habits of the person as anomalies in the daily life of the user with the Isolation Forest method. Furthermore, we show an application for the identification of food-related scenes when the camera wearer eats in isolation. Results have shown the good performance of the proposed model and its relevance to visualize the nutritional habits of individuals.

==> isolation.tex <==
\begin{table}[H]
\centering
 \scalebox{1}{
\resizebox{\columnwidth}{!}{\begin{tabular}{l|l|l|l|l|l|l|l|l}
& \multicolumn{2}{c}{ Total scenes } & \multicolumn{2}{c}{ Total food scenes } & \multicolumn{2}{c}{ Total isolated scenes } & \multicolumn{2}{c}{ \% of isolated scenes } \\
\hline
\hline
User 1 & \multicolumn{2}{c}{ 20543 } & \multicolumn{2}{c}{ 2777 } & \multicolumn{2}{c}{ 286 } & \multicolumn{2}{c}{ 0.103 } \\
User 2 & \multicolumn{2}{c}{ 11815 } & \multicolumn{2}{c}{ 2377 } & \multicolumn{2}{c}{ 292 } & \multicolumn{2}{c}{ 0.123 } \\
User 3 & \multicolumn{2}{c}{ 21625 } & \multicolumn{2}{c}{ 5061 } & \multicolumn{2}{c}{ 899 } & \multicolumn{2}{c}{ 0.178 } \\
User 4 & \multicolumn{2}{c}{ 18977 } & \multicolumn{2}{c}{ 5378 } & \multicolumn{2}{c}{ 571 } & \multicolumn{2}{c}{ 0.107 } \\
User 5 & \multicolumn{2}{c}{ 17046 } & \multicolumn{2}{c}{ 5731 } & \multicolumn{2}{c}{ 702 } & \multicolumn{2}{c}{ 0.123 } \\
User 6 & \multicolumn{2}{c}{ 16592 } & \multicolumn{2}{c}{ 3512 } & \multicolumn{2}{c}{ 326 } & \multicolumn{2}{c}{ 0.093 } \\
User 7 & \multicolumn{2}{c}{ 11207 } & \multicolumn{2}{c}{ 3497 } & \multicolumn{2}{c}{ 323 } & \multicolumn{2}{c}{ 0.093 } \\
\end{tabular}}
}
\caption{Number of isolated food scenes (i.e. instances of eating in front of the computer or the TV) as compared to the total number of food scenes and total number of recorded scenes for the users from the \textit{EgoRoutine} data set.}
\label{table:isolation}
\end{table}
